HIVE: Scalable Hardware-Firmware Co-Verification using Scenario-based Decomposition and Automated Hint Extraction

Hardware-firmware co-verification is critical to design trustworthy systems. While formal methods can provide verification guarantees, due to the complexity of firmware and hardware, it can lead to state space explosion. There are promising avenues to reduce the state space during firmware verification through manual abstraction of hardware or manual generation of hints. Manual development of abstraction or hints requires domain expertise and can be time-consuming and error-prone, leading to incorrect proofs or inaccurate results. In this paper, we effectively combine the scalability of simulation-based validation and the completeness of formal verification. Our proposed approach is applicable to actual firmware and hardware implementations without requiring any manual intervention during formal model generation or hint extraction. To reduce the state space complexity, we utilize both static module-level analysis and dynamic execution of verification scenarios to automatically generate system-level hints. These hints guide the underlying solver to perform scalable equivalence checking using proofs. The extracted hints are validated against the implementation before using them in the proofs. Experimental evaluation on RISC-V based systems demonstrates that our proposed framework is scalable due to scenario-based decomposition and automated hint extraction. Moreover, our fully automated framework can identify complex bugs in actual firmware-hardware implementations.

==> Images/case2.tex <==
\begin{minted}
[
% frame=lines,
% framesep=2mm,
% baselinestretch=1.2,
fontsize=\footnotesize,
linenos,
xleftmargin=2em,
]
{c}
#include <stddef.h>
#include "driver.h" 

#define BUFFER_SIZE 128

int main(void) {
    char buffer[BUFFER_SIZE];
    uart_init(); // Initialize UART
    while(1) {
        memset(buffer, 0, sizeof(buffer)); // Clear buffer
        uart_read(buffer, BUFFER_SIZE); // Read from UART   
    }
    return 0;
}
\end{minted}

==> Images/case3.tex <==
\begin{minted}
[
% frame=lines,
% framesep=2mm,
% baselinestretch=1.2,
fontsize=\footnotesize,
linenos,
xleftmargin=2em,
]
{c}
#include <stddef.h>
#include "tlcontroller.h" 

int main(void) {
    // Traffic sensor in side street triggered
    tlc_request_side(); // request side street green
    return 0;
}
\end{minted}

==> Images/case4.tex <==
\begin{minted}
[
% frame=lines,
% framesep=2mm,
% baselinestretch=1.2,
fontsize=\footnotesize,
linenos,
xleftmargin=2em,
]
{c}
#include <stddef.h>
#include "tlcontroller.h" 

int main(void) {
    //Pedestrian request received to cross the road
    tlc_request_cross(); //pedestrian crossing light
    return 0;
}
\end{minted}

==> Images/concretize_sample.tex <==
\begin{minted}
[
% frame=lines,
% framesep=2mm,
% baselinestretch=1.2,
fontsize=\footnotesize,
linenos,
xleftmargin=2em,
]
{racket}
(define (concretize-case1 module)
    (match module
        [`uart (for ([field (list 
                    "count_cycle" 
                    "count_instr"
                    "send_divcnt"
                    ... )])
                (match-abstract! field field))]
        [`cpu (for ([field (list 
                    ... )])
                (match-abstract! field field))]
        ....
        [default (displayln "Module not found!")]))
 
; Usage of hints in the proofs
(require "symcrete/dut/hints.rkt") ; import hints
(hint concretize-case1 `uart) ; use for UART proof
\end{minted}

==> Images/hint1.tex <==
\begin{minted}
[
% frame=lines,
% framesep=2mm,
% baselinestretch=1.2,
fontsize=\footnotesize,
% linenos,
% xleftmargin=2em,
]
{racket}
(define (hints method c1 f1 f-out f2)
  (match method
    ['(pop)
     (make-hintdb
      [split-has-data
       (tactic
        (define have-data (equal? 
            (get-field c1 'have_data) (bv 1 1)))
        (case-split! (list have-data (! have-data)))
        (concretize! (lens 'circuit 'have_data)))])]
    [_ #f]))
\end{minted}

==> sections/comments.tex <==
\newpage

\section{Responses to Reviewer Comments}
We would like to thank the reviewers for their thorough and insightful comments. We have modified the manuscript to address various issues raised by the reviewers. This section outlines all the reviewer comments and our responses in terms of how we have addressed the issues in the modified manuscript. The modifications are marked in blue.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{REVIEWER 1}

\begin{noindlist}


\item The current evaluation is limited to three small benchmark circuits. Expanding these evaluations to include real-world, complex designs would be beneficial in assessing the scalability of the proposed approach.

\color{blue}
 \vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. Note that the three benchmarks are real-life embedded systems. They are full-system implementations and widely used for various application domains. We have also added a new benchmark, a mass storage controller SoC, to demonstrate the scalability and applicability of our proposed approach.

\begin{figure}[H]
    \begin{center}
    \vspace{-0.1in}
    % \begin{adjustwidth*}{-1em}{-1em}
        % \footnotesize
        % \small
        \input{Images/satasoc}
    % \end{adjustwidth*}
    \end{center}
      % \vspace{-0.1in}
      \caption{\color{blue}SoC that integrates SATA controller to communicate with the mass storage device.}
        \vspace{-0.1in}
      \label{fig:sataSoC1}
\end{figure}

\textbf{\textit{Case Study 4: Mass Storage (SATA) Controller}}: Serial Advanced Technology Attachment (SATA) controller is a hardware module that manages the communication between a SoC and mass storage devices (such as hard disk drives and solid-state drives). In this case study, we have utilized a SATA controller that connects to the SoC using the AXI (Advanced eXtensible Interface) as illustrated in Figure~\ref{fig:sataSoC1}. The controller is configured and managed by the firmware driver, which has the ability to change the state of the data transfer between the mass storage device attached to the controller based on the requirement of the application code. For simulation purposes, we have used the Verilog \texttt{readmemb}  function as the mass storage device.

\begin{table}[H]
\centering
\small
\caption{\color{blue}Time (in Minutes) and memory (in Megabytes) consumed by the verification process of the SoC with the SATA device connected via SATA controller for different verification scenarios of \textit{SATA controller}. \textit{We did not show comparison with state-of-the-art since existing methods without hints face timeouts for all scenarios.}}\label{tab:SATAresults1}
\vspace{-0.05in}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|cc|cc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Test Cases for\\ SATA Driver\end{tabular}}}} & \multicolumn{2}{c|}{\textbf{Hint Generation}} & \multicolumn{2}{c|}{\textbf{Equival. Checking}} \\ \cline{2-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textbf{Time}} & \multicolumn{1}{c|}{\textbf{Memory}} & \multicolumn{1}{c|}{\textbf{Time}} & \multicolumn{1}{c|}{\textbf{Memory}} \\ \hline
\textit{Initialization Sequence} & \multicolumn{1}{c|}{39} &  3109& \multicolumn{1}{c|}{274} & 2850 \\ \hline
\textit{Handshake Phase} & \multicolumn{1}{c|}{41} & 3190 & \multicolumn{1}{c|}{269} & 2689 \\ \hline
\textit{Command Phase} & \multicolumn{1}{c|}{43} & 3019 & \multicolumn{1}{c|}{255} & 2503 \\ \hline
\textit{RX Transaction} & \multicolumn{1}{c|}{34} &  3100 & \multicolumn{1}{c|}{270} & 2476 \\ \hline
\textit{TX Transaction} & \multicolumn{1}{c|}{34} &  3100 & \multicolumn{1}{c|}{270} & 2476 \\ \hline
\end{tabular}}
\vspace{-0.1in}
\end{table}

The firmware driver is responsible for managing the SATA controller to perform handshake, establishing and maintaining the communication protocol between the system and the storage device, thereby ensuring reliable and synchronized data exchange. SATA controller implementation consists of several nested FSMs in order to achieve the above functionalities. In order to evaluate the effectiveness of \textit{HIVE}, we have selected several functional scenarios from the implementation. These functional scenarios include testing the controller initialization, SATA handshake, controller commands, and read and write transactions. Table~\ref{tab:SATAresults1} presents the elapsed time and consumed memory for hint generation as well as verification with \textit{HIVE}.






\color{black}


\color{black}
 \vspace{0.1in}

\item The introduction can further highlight the differentiation w.r.t simulation-based dynamic verification techniques. The authors could expand the introduction by 1-2 sentences to better distinguish their technique from existing simulation-based validation approaches. Specifically, highlighting the limitations of simulation coverage and input space complexity will motivate the need for formal techniques that can provide exhaustive verification. The authors can then contrast how their automated hint-driven formal flow can scale verification compared to standard formal methods that also face state space explosion issues. This will help strengthen the problem motivation.


\color{blue}
 \vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. We have added the following discussion to the introduction.

\vspace{0.05in}
Simulation-based validation provides the ability to simulate the design using input stimuli and validate whether the particular input can produce the expected output by concretizing values corresponding to the unrelated components. However, it can only provide guarantees for that particular input. On the other hand, symbolic simulation allows the designs to be simulated with all possible inputs while monitoring for contradiction cases, however, it can lead to state space explosion. We effectively combine the best of both worlds to achieve the objective of HIVE. In other words, the design slicing feature of concrete simulation-based validation is combined with symbolic simulation to formally evaluate the implementation against target verification scenarios.


\color{black}
 \vspace{0.1in}

\item Certain parts like Section III-G seem abrupt without sufficient connection to the overall flow. More transitions are needed. Some sections like III-G introduce new concepts quite abruptly without explaining the logical connection to previous sections. For example, III-G discusses symbolic execution limitations and mitigation using hints, but this seems disconnected from the earlier sections. Adding smoother transitions that relate the concepts or provide previews of upcoming topics would improve overall flow understanding and continuity.


\color{blue}
 \vspace{0.1in}
\noindent \textbf{Response:} Thank you for the comment. We have added the following lines to the discussion to enable a smooth transition. 


\vspace{0.05in}
So far we have discussed the process of automatically generating hints. In this section, we describe the steps to convert the implementation into a formal model and how the generated hints are utilized to address the path explosion. For this purpose, we convert a copy of the system model with inline firmware application (without test scenarios) to SMT format, which serves as our formal model for equivalence checking. 


\color{black}
 \vspace{0.1in}
 



\end{noindlist}

\subsection{REVIEWER 2}

\begin{noindlist}
\item  I would like to thank the authors for making the revision and addressing my questions. I have no more concerns for this paper.

\color{blue}
 \vspace{0.1in}
\noindent \textbf{Response:}
Thank you for the comment. 

\color{black}
 

\end{noindlist}


\subsection{REVIEWER 3}

\begin{noindlist}

 
\item  Thanks for addressing the comments in the previous round of review and resubmitting. I do not have additional questions or comments.


\color{blue}
 \vspace{0.1in}
\noindent \textbf{Response:}
Thank you for the comment. 

\color{black}
 



\end{noindlist}


